Attack as Defense: Characterizing Adversarial Examples using Robustness

As a new programming paradigm, deep learning has expanded its application to many real-world problems. At the same time, deep learning based software are found to be vulnerable to adversarial attacks. Though various defense mechanisms have been proposed to improve robustness of deep learning software, many of them are ineffective against adaptive attacks. In this work, we propose a novel characterization to distinguish adversarial examples from benign ones based on the observation that adversarial examples are significantly less robust than benign ones. As existing robustness measurement does not scale to large networks, we propose a novel defense framework, named attack as defense (A2D), to detect adversarial examples by effectively evaluating an example's robustness. A2D uses the cost of attacking an input for robustness evaluation and identifies those less robust examples as adversarial since less robust examples are easier to attack. Extensive experiment results on MNIST, CIFAR10 and ImageNet show that A2D is more effective than recent promising approaches. We also evaluate our defence against potential adaptive attacks and show that A2D is effective in defending carefully designed adaptive attacks, e.g., the attack success rate drops to 0% on CIFAR10.

==> attack-defense.tex <==

\section{Representative Adversarial Attacks and Defense}\label{sec:attack-defense}
We briefly review some representative adversarial attack methods which will be used in this work.\jy{We need to choose several representative attacks for this paper, also should we move the threat model here?}
\fu{Not sure do we really need this section!}

\smallskip
\noindent \textbf{FGSM}: The Fast Gradient Sign Method (FGSM)~\cite{FGSM15}
looks for a similar sample $\Hat{x}$ of the input $x$ that
fools the target NN.
FGSM uses a cost function $\mathbf{J}(x,c_x)$ that
describes the cost of classifying $x$ as label $c_x$
and  transforms the problem to maximize the cost function.
The optimization problem is solved by performing one step gradient update from the input $x$
with an $L_\infty$ distance threshold $\epsilon$.
Formally, a potential adversarial example $\Hat{x}$ could be crafted
as follows:
\[
    \Hat{x}=x+{\epsilon}\times\mathbf{sign}(\nabla_x{\mathbf{J}(x,c_x)}),
\]
%is designed based on the intuition that a NN can largely be fooled by changing the softmax value of each input to the largest extent, which is represented by its gradient.
% explanation of the neural networks vulnerability that it is its linear nature that makes a neural network easy to be misled instead of the nonlinearity and over?tting. If the softmax score of a class linearly has to do with the input, we could just linearly modify
% the input to make the softmax score of the true label decrease.
% With,
 %By simply adding up the sign of gradient of the cost function with respect to the input $x$, a potential adversarial example $\Hat{x}$ could be crafted
%as follows:
%\[
%    \Hat{x}=x+{\epsilon}\times\mathbf{sign}(\nabla_x{\mathbf{J}(x,c_x)}),
%\]
where %$\mathbf{J}(x,c_x)$ is the cost used to train the model,
$\nabla_x{\mathbf{J}(x,c_x)}$ is the gradient of $\mathbf{J}(x,c_x)$,
and $\mathbf{sign}(\cdot)$ is a sign function such that $\mathbf{sign}(c)=+1$ if $c>0$, $\mathbf{sign}(c)=-1$ if $c<0$ and $\mathbf{sign}(c)=0$ if $c=0$.

Thought this attack is simple and fast, it does not guarantee that (1) $\Hat{x}$ must be an adversarial example or (2) the adversarial perturbation is minimal even if $\Hat{x}$ is an adversarial example.

\smallskip
\noindent \textbf{BIM}:
Iterative gradient sign Method (BIM) is an iterative version of FGSM~\cite{KGB17}.
For each iteration, BIM performs FGSM with a small step size $\alpha$
and clips the result so that it stays in the $\epsilon$-neighbourhood of the input sample.
The $i$th iteration is updated by as follows: ($x^0=x$)
\[
   x^{i+1}={\tt clip}_{\epsilon,x}(x^i+\alpha\times\mathbf{sign}(\nabla{\mathbf{J}(x,c_x)})).
\]
This update can be used for both $L_2$ and $L_\infty$.
Such iteration is then repeated for several
times which greatly improves the success rate of FGSM attack.

% though it is an efficient manner.
\smallskip
\noindent \textbf{JSMA}: Jacobian-based Saliency Map Attack (JSMA)~\cite{JSMA} is devised to attack a NN model with minimal perturbations.
 JSMA aims to craft an adversarial sample for each input so that adversarial sample is misclassified to a certain (attacker-chosen) label by the target NN.
 It is based on a greedy algorithm that changes one pixel during each iteration to increase the probability of having the target label.
 The idea is to calculate a saliency map based on the Jacobian matrix to model the impact that each pixel imposes on the classification.
 Formally, assume that  the last layer of $f$ is the softmax function and the inputs to the softmax function
are called logits. Let $\mathbf{F}$ denote the function of the NN $f$ excluding the softmax function (i.e., the logits), and $\mathbf{F}_k$ denotes
 the function of $\mathbf{F}$ with respect to the logit $k$.
 The saliency map $S(x,t)$ at each iteration is defined as follow: for the input $x$ and a logit $t$ that corresponds the target label,
\[ S(x,t)_i =  \left\{
   \begin{array}{ll}
     a_i\times\left|b_i\right|, & \mbox{if} \ a_i>0 \ \mbox{and} \ b_i<0; \\
     0, & \mbox{otherwise}.  \\
   \end{array}
   \right. \]
   where $i$ is an input feature, $a_i = \frac{\partial{\mathbf{F}_t(x)}}{\partial{x_i}}$ and $b_i =  \sum_{k \neq t}\frac{\partial{\mathbf{F}_k(x)}}{\partial{x_i}}$ with $k$ being other logits.

 With the saliency map $S(x,t)$, it picks a pixel which may have the most significant influence on the desired label and then increases it to the maximum value. The process is repeated until it reaches one of the termination criteria, i.e., the number of modified pixels has reached the bound, or the target label has been achieved.

%\[\mbox{Defining } \left\{
%    \begin{aligned}
%       a_i = & \frac{\partial{\mathbf{F_t}(x)}}{\partial{X_i}},\\
%       b_i = & \sum_{k \neq t}\frac{\partial{\mathbf{F_k}(x)}}{\partial{X_i}},
%    \end{aligned}
%\right.\]


However, it is too strict to select one pixel at a time because few pixels could meet that definition. Thus, instead of picking one pixel per iteration, the authors proposed to pick two
pixels to modify per iteration according to the follow objective:
\[
\arg\max_{(p_1,p_2)} \left(\sum_{i\in\{p_1,p_2\}} \frac{\partial{\mathbf{F}_t(x)}}{\partial{x_i}}\right)\times \left|\sum_{i\in\{p_1,p_2\}} \ \sum_{k \neq t} \frac{\partial{\mathbf{F}_k(x)}}{\partial{x_{i}}}    \right|
\]
where $(p_1,p_2)$ is the candidate pair of pixels.

JSMA is relatively time-consuming and memory-consuming since it needs to compute the Jacobian matrix and picks out a pair from nearly $\binom{n}{2}$ candidate pairs at each iteration, where
$n$ denotes the number of pixels.

% Remind, there is a decreased-counterpart of the saliency map defined above, but they are
\smallskip
\noindent \textbf{DeepFool}:
The authors of Deepfool assume that the neural
networks are totally linear, with a hyperplane separating each
class from another~\cite{DeepFool}. Based on this assumption,
DeepFool is to make the benign samples cross the decision boundary with minimal perturbations~\cite{DeepFool}.
However, in practice,  neural networks are not totally linear.
To address this problem, DeepFool adopts an iterative algorithm which iteratively uses the above idea to craft a sample.
 The exact derivation process is complicated and thus we refer the readers to~\cite{DeepFool} for details.

\smallskip
\noindent \textbf{C\&W}:
Carlini \emph{et al.}~\cite{CW} proposed a group of attacks based on three distance metrics. The key idea is to solve an optimization problem which minimizes the perturbation imposed on the benign sample (with certain distance metric) and maximizes the probability of the target class label.
% Note, JSMA minimizes the perturbations by restricting the number of pixels which need to be changed while C\&W does this by minimizing the total changes of all pixels.
% They designs a series of loss functions to make the desired class's probability as large as possible.
The objective function is as follow:
\[
    \arg\min \Delta x + c\cdot f(\hat{x},t)
\]
where $\Delta x$ is defined according to some distance metric, e.g, $L_0$, $L_2$ and $L_{\infty}$ norms, $\hat{x}=x+\Delta x$ is the clipped adversarial sample and $t$ is its target label. The idea is to devise a clip function for the adversarial sample such that the value of each pixel dose not exceed the legal range. The clip function and the best loss function according to~\cite{CW}  are shown as follows.
\begin{equation}
\begin{aligned}
{\tt clip}:& \ \hat{x} &=& 0.5(tanh(\tilde{x})+1) \\ \nonumber
{\tt loss}:&  \ f(\hat{x},t) &=& \max(\max\{G(\hat{x})_c:c \neq t\}-G(\hat{x})_t, \neg \kappa)
\end{aligned}
\end{equation}
where $G(x)$ denotes the output vector of the target NN, $t$ is the target class,
$\kappa$ is a hyper-parameter
called confidence. Higher confidence often results in adversarial examples that are stronger in classification confidence.
Readers can refer to~\cite{CW} for details.

% $\gamma$ is an hyperparameter which encourages the solver to ?nd an adversarial samples with high con?dence.

All the above mentioned attacks are white-box attacks which means that the attackers require the full knowledge of the DNN model.
There do exist black-box attacks that the adversary only needs to know the output of the DNN model for each input.
One black-box attack is to train a substitute model to mimic the behaviors of the target model with data augmentation. Then, it applies one of the existing attack algorithm, e.g., FGSM and JSMA, to generate adversarial samples for the substitute model. The key assumption to its success is that the adversarial samples transfer between different model architectures~\cite{Intriguing,FGSM15}.

% \noindent {\bf Defense Related Work}.
% The current defense strategies against adversarial samples can be divided into three main categories, i.e., model modification, input transformation and detection.

% \noindent {\bf Model Modification.}

% \noindent {\bf Input Transformation.} This kind of defense strategies try to secure the model by preprocessing the input samples at inference time before they are fed to the model for recognition. Formally speaking, a preprocessor $g(\cdot)$ is added in front of the model $f(\cdot)$. Some preprocessores are non-differentiable, such as JPEG compression~\cite{guo}, image quilting~\cite{guo},
% % Advantage (stand alone); Disadvantage (easily bypassed by adaptive attack, especially those differentiable); retrain f() on transformed data to increase accuracy on benign samples.

% \noindent {\bf Detection.}

